Weakly-Supervised Multi-Face 3D Reconstruction

3D face reconstruction plays a very important role in many real-world multimedia applications, including digital entertainment, social media, affection analysis, and person identification. The de-facto pipeline for estimating the parametric face model from an image requires to firstly detect the facial regions with landmarks, and then crop each face to feed the deep learning-based regressor. Comparing to the conventional methods performing forward inference for each detected instance independently, we suggest an effective end-to-end framework for multi-face 3D reconstruction, which is able to predict the model parameters of multiple instances simultaneously using single network inference. Our proposed approach not only greatly reduces the computational redundancy in feature extraction but also makes the deployment procedure much easier using the single network model. More importantly, we employ the same global camera model for the reconstructed faces in each image, which makes it possible to recover the relative head positions and orientations in the 3D scene. We have conducted extensive experiments to evaluate our proposed approach on the sparse and dense face alignment tasks. The experimental results indicate that our proposed approach is very promising on face alignment tasks without fully-supervision and pre-processing like detection and crop. Our implementation is publicly available at \url{https://github.com/kalyo-zjl/WM3DR}.

==> fig_qualitative.tex <==
\begin{figure*}
%\begin{tabular}{cccccccc}
\begin{tabular}{cc@{\hspace{0mm}}c@{\hspace{0mm}}c@{\hspace{0mm}}c@{\hspace{0mm}}c@{\hspace{0mm}}c@{\hspace{0mm}}}
% Inputs
\vspace{.4em}
\hspace{-0.7cm}{Input} &
\includegraphics[width=0.75in,align=c]{full-qual/in/02.png} &
\includegraphics[width=0.75in,align=c]{full-qual/in/16.png} &
\includegraphics[width=0.75in,align=c]{full-qual/in/03.png} &
\includegraphics[width=0.75in,align=c]{full-qual/in/49.png} &
\includegraphics[width=0.75in,align=c]{full-qual/in/11.png} &
\includegraphics[width=0.75in,align=c]{full-qual/in/29.png}\\

% Us
\vspace{.4em}
% Revision: nov8, from large set.
\hspace{-0.7cm}{Ours} &
\includegraphics[width=0.8in,align=c]{full-qual/us/02.png} &
\includegraphics[width=0.8in,align=c]{full-qual/us/16.png} &
\includegraphics[width=0.8in,align=c]{full-qual/us/03.png} &
\includegraphics[width=0.8in,align=c]{full-qual/us/49.png} &
\includegraphics[width=0.8in,align=c]{full-qual/us/11.png} &
\includegraphics[width=0.8in,align=c]{full-qual/us/29.png}\\

% Us
\vspace{.4em}
% Revision: nov8, from large set.
\hspace{-0.7cm}{Genova et al.} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/02.png} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/16.png} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/03.png} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/49.png} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/11.png} &
\includegraphics[width=0.75in,align=c]{full-qual/genova/29.png}\\

% Tran
\vspace{.4em}
\hspace{-0.7cm}{Tran\cite{tran2017regressing}} &
%\cite{tran2017regressing} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/02.png} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/16.png} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/03.png} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/49.png} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/11.png} &
\includegraphics[width=0.75in,align=c]{full-qual/tran/29.png}\\

% MoFA
\vspace{.4em}
\hspace{-0.7cm}{MoFA\cite{tewari17MoFA}} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/02.png} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/16.png} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/03.png} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/49.png} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/11.png} &
\includegraphics[width=0.75in,align=c]{full-qual/mofa/29.png}\\

\end{tabular}
\caption{Results on the MoFA-Test dataset. Our method shows improved likeness and color fidelity over competing methods, especially in the shape of the eyes, eyebrows, and nose. Note that MoFA~\cite{tewari17MoFA}  solves for pose, expression, lighting, and identity, so is shown both with (row 5) and without (row 4) expression. The unstructured method of Sela, et al.~\cite{sela2017unrestricted} produces only geometry, so is shown without color.}
\label{fig:qualitative}
\end{figure*}
